MUG: Interactive Multimodal Grounding on User Interfaces

We present MUG, a novel interactive task for multimodal grounding where a user and an agent work collaboratively on an interface screen. Prior works modeled multimodal UI grounding in one round: the user gives a command and the agent responds to the command. Yet, in a realistic scenario, a user command can be ambiguous when the target action is inherently difficult to articulate in natural language. MUG allows multiple rounds of interactions such that upon seeing the agent responses, the user can give further commands for the agent to refine or even correct its actions. Such interaction is critical for improving grounding performances in real-world use cases. To investigate the problem, we create a new dataset that consists of 77,820 sequences of human user-agent interaction on mobile interfaces in which 20% involves multiple rounds of interactions. To establish our benchmark, we experiment with a range of modeling variants and evaluation strategies, including both offline and online evaluation-the online strategy consists of both human evaluation and automatic with simulators. Our experiments show that allowing iterative interaction significantly improves the absolute task completion by 18% over the entire test dataset and 31% over the challenging subset. Our results lay the foundation for further investigation of the problem.

==> analysis.tex <==
\section{Analysis} \label{sec:anlysis}

Tab.~\ref{tab:dup_analysis} shows how model predictions are affected by corrective instructions generated by heuristics or the neural instruction model.
On the challenging subset, there are about half of examples where our agent models make repeatedly the same incorrect selection, irrespective of the corrective instruction.
Even considering the entire test set, there are still $\geq26\%$ such cases.
We broadly attribute this observation to the difficulty of the task as well as the challenge in multimodal modeling.

\begin{table}[ht]
\small
\def\arraystretch{1}
  \centering
  \scalebox{1}{
  \begin{tabular}{l|c|c!{\vrule width 1pt}c|c}
    \toprule
    & \multicolumn{2}{c!{\vrule width 1pt}}{Challenging} & \multicolumn{2}{c}{All} \\
    \midrule
    & {Heuristics} & {Neural} & {Heuristics} & {Neural} \\
    \midrule
    Single & 57.8 & 56.6    & 33.4 & 34.0 \\
    Ins-only & 48.4 & 53.3  & 27.0 & 30.4 \\
    Multi & 49.5 & 52.9     & 27.4 & 30.6 \\
    Imitation & 57.8 & \tb{45.3}    & 26.6 & \tb{26.2} \\
    RL & \tb{47.3} & 50.8 & \tb{26.0} & 29.0 \\
    \bottomrule
  \end{tabular}}
  \caption{Percentage of example have duplicated predictions across turns. Lower values indicates more sensitive to user instructions.}~\label{tab:dup_analysis}
\end{table}

\begin{table}[ht]
\small
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1}
  \centering
  \scalebox{0.98}{
  \begin{tabular}{l|c|c|c|c|c|c}
    \toprule
    {\emph{Multi}} & {\foneat{0}} & {\foneat{1}} & {\foneat{2}} & {\foneat{3}} & {\foneat{4}} & {\%Dup}$\downarrow$ \\
    \midrule
    Heuristics & 25.2 & \tb{47.8} & \tb{50.9} & \tb{51.7} & \tb{52.4} & \tb{49.5} \\
    Random & 25.2 & 34.0 & 37.4 & 38.2 & 38.6 & 62.7 \\
    Reuse 1st & 25.2 & 29.3 & 30.9 & 31.6 & 32.0 & 70.2 \\
    \bottomrule
  \end{tabular}}
  \caption{Heuristics v.s. immediate alternatives on the \emph{Challenging} split using the \emph{Multi} model.
  \emph{Random}: instruction templates instantiated with random target object on the interface.
  \emph{Reuse 1st}: reusing the first instruction across turns.}~\label{tab:random_heuristics}
\end{table}

Tab.~\ref{tab:random_heuristics} compares our heuristics-based online evaluation against immediate alternatives.
The large and consistent performance gaps suggest our agent model follows the hints in corrective instructions instead of making blind guesses across turns.
For brevity, we used the \emph{Multi} model to demonstrate.
Other multi-turn models performed in a similar pattern (e.g., consistently $15\sim20\%$ better \foneat{4} when using Heuristics).


==> limitations.tex <==
\section{Limitations}
\paragraph{English-only Dataset}
While non-English examples exists, we acknowledge that \myname mostly consists of English UI.
Specifically, our instructions are English-only.
Future extensions to our work should address or alleviate this issue.

\paragraph{Platform-specific Interfaces}
Our interfaces, since coming from RICO, only consist of Android screens.
In practice, it is also difficult to obtain non-Android interfaces.
We acknowledge this is an application limitation.
And the bias from the top and bottom banner of Android could make trained model brittle in other domains.

\paragraph{Limited to a Single Screen}
\myname focues on correcting agent actions within the same user interface.
A natural extension would be adapting the task to span over sequence of interfaces.
Indeed, the task would become more challenging, and potentially require large offline training data and reliable online simulation.

\paragraph{Better User Model}
The current best neural instruction generation we use has a CIDEr $78.0$ on the validation set.
We acknowledge there is space for further improvement.
Note that our neural instructions are trained on multi-turn examples in \myname, which amounts to $\sim20\%$ of the training data.
It suggests external resources could be useful for improving user model performances.

\paragraph{Agent Mistakes}
It would helpful to study how/why the agent sometime repeatedly makes incorrect actions in Tab.~\ref{tab:dup_analysis}.
This would help improve model robustness and mitigate the impact from potential data artifact.
